MAP4CS: A Multi-dimensional Data Pruning Framework for Efficient Code Retriever Fine-tuning

Retrieval-Augmented Generation (RAG) has become a cornerstone in software engineering for enhancing Large Language Models (LLMs) with domain-specific knowledge. However, adapting retrievers to evolving code repositories remains challenging due to the noise and redundancy inherent in massive code corpora. Standard fine-tuning on the full corpus is computationally expensive and often leads to sub-optimal performance due to negative transfer from low-quality samples. Conversely, simple random sampling fails to guarantee data representativeness. To address these challenges, we propose MAP4CS (Multi-dimensional Awareness Pruning for Code Search), an adaptive data pruning framework. MAP4CS identifies a small, high-quality core subset by integrating syntactic structure, semantic diversity, and distributional representation, followed by a rigorous rule-based filtering pipeline. Extensive experiments on two large-scale datasets demonstrate that MAP4CS consistently outperforms random sampling baselines using only 5% of the training data. Remarkably, it achieves performance comparable to, or even superior to, fine-tuning on the full dataset, validating the ''less is more'' hypothesis in data-centric AI. Furthermore, linguistic analysis reveals an adaptive optimization mechanism: MAP4CS automatically functions as a de-duplicator for redundant corpora and a denoiser for chaotic ones, constructing a training corpus that is both lexically diverse and information-dense.

==> sections/5_Result/RQ4.tex <==
% \vspace{-10pt}
\subsection{RQ4: Impact of Self-evolution}

To evaluate the impact of the self-evolution process on \ourapproach, we design three knowledge base stages—0\%, 50\%, and 100\%—to simulate different stages of self-evolution. Here, 0\% corresponds to the baseline (LLM-based with Prompt Engineering), and 100\% corresponds to \ourapproach.
To comprehensively assess the practicality of the self-evolution process in different translation scenarios and to account for the randomness in the translation order of the target functions, we construct 50\% knowledge base as follows:
Dependency usage examples: For each target function, we randomly retain 50\% of the dependency usage examples available at the 100\% stage. The remaining 50\% dependencies have their dependency usage examples set to empty, representing no reference is available in current project’s context.
Target-language Code Samples: We randomly select 50\% projects from the collected projects and extract functions to construct the samples.
Successful translation function pairs: For each target function, we randomly select 50\% of the successful translation function pairs available at the 100\% stage. These selected pairs are then used as candidates for the top-1 successful translation function pair retrieval.

As shown in Table~\ref{tab:rq4_result}, when the knowledge base expands from 0\% to 50\%, execution-based metrics show significant improvements: Compilation@1, Pass@1, and DSR@1 increase by 11.7\%, 12.5\%, and 6.7\%, respectively, despite a slight decrease in Repairable Ratio. Similarly, match-based metrics exhibit substantial growth, with CodeBLEU increasing from 0.604 to 0.695 and \astmatchscore from 0.401 to 0.507.
When the knowledge base further expands from 50\% to 100\%, translation performance continues to improve, with relative improvement in various metrics ranging between 5.5\% and 16.4\%. As previous analyzed, the self-evolution process significantly enhances translation performance in both stages (0\% to 50\% and 50\% to 100\%). However, the improvements from 50\% to 100\% are less pronounced compared to the initial stage (0\% to 50\%). This suggests that after reaching 50\%, the remaining challenges may not be fully addressed through knowledge-driven enhancements alone, which we will explore in detail in RQ5 (Section \ref{sec:rq5}).

\finding{As the self-evolution process progresses, the knowledge base continuously enhances the LLM’s performance across various aspects of the repository-level code translation.}



==> sections/5_Result/RQ5.tex <==
% \vspace{-10pt}
\subsection{RQ5: \colortext{Case Study}}
\label{sec:rq5}

To fully understand the advantages and limitations of \ourapproach, we further manually analyze the successful examples of \ourapproach that the baselines fail, and the failure examples of \ourapproach.

\begin{table}[tp]
% \vspace{-10pt}
\caption{The Number of Top3 Error Causes of Dependencies Misuse of \ourapproach and LLM-based Baseline}
\centering
\begin{adjustbox}{width=0.85\linewidth}
        \begin{tabular}{@{}c|c|ccc}
            \hline
            \multirow{2}{*}{\textbf{Model}}  & \multirow{2}{*}{\textbf{Tech.}} & \multicolumn{3}{c}{\textbf{Error type}}                   \\ \cline{3-5} 
            & & \begin{tabular}[c]{@{}l@{}}\textbf{Function Differences}\\\textbf{Misinterpretation ↓}\end{tabular}  & \begin{tabular}[c]{@{}l@{}}\textbf{Data Type Differences}\\ \textbf{Misinterpretation ↓}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Variable Differences}\\\textbf{Misinterpretation ↓}\end{tabular} \\ \hline


            
            \multirow{3}{*}{\claude} 
            & Basic RAG             & 368         & 2    & 131   \\ 
            & PE                    & \textbf{191}         & \textbf{0}    & 58   \\ 
            & \textbf{\ourapproach} & 247         & \textbf{0}    & \textbf{40}   \\ \hline
            \multirow{3}{*}{\rdeepseek}  
            & Basic RAG             & 228         & 1      & 48 \\ 
            & PE                    & \textbf{172}         & \textbf{0}      & 32\\
            & \textbf{\ourapproach} & 256         & 2      & \textbf{24}   \\ \hline
            \multirow{3}{*}{\vdeepseek}  
            & Basic RAG             & 420         & 1      & 188 \\ 
            & PE                    & 368         & \textbf{0}      & 100  \\
            & \textbf{\ourapproach} & \textbf{338}         & \textbf{0}      & \textbf{62}    \\ \hline
            \multirow{3}{*}{\qwenthreetwo}  
            & Basic RAG             & 679         & 11     & 220  \\ 
            & PE                    & 677         & 7      & 162  \\
            & \textbf{\ourapproach} & \textbf{447}         & \textbf{2}      & \textbf{83}   \\ \hline
            \multirow{3}{*}{\qwenfourteen} 
            & Basic RAG             & 1,288        & 11     & 219   \\ 
            & PE                    & 1,400        & 9      & 137 \\ 
            & \textbf{\ourapproach} & \textbf{524}         & \textbf{0}      & \textbf{64}   \\ \hline

            \multirow{3}{*}{Total} 
            & Basic RAG             & 2,983       & 25      & 806   \\ 
            & PE                    & 2,809       & 17      & 489 \\ 
            & \textbf{\ourapproach} & \textbf{1,812}       & \textbf{4}       & \textbf{273}   \\ \hline
            
        \end{tabular}
        \end{adjustbox}
\label{tab:rq5_case_study_good_case_compare_with_llm-based_baseline}
% \vspace{-10pt}
\end{table}

\subsubsection{Analysis of Successful Examples}
Since LLM translation failures on RustRepoTrans are attributed to Dependencies Misuse errors in as high as 77.9\% of cases~\cite{ou2024repository}, we statistically analyzed the top three categories of Dependencies Misuse errors in the translation results of \ourapproach and all baselines:  
Function Differences Misinterpretation, Data Type Differences Misinterpretation, and Variable Differences Misinterpretation, recording the specific count for each category.

In terms of LLM-based baselines, as shown in Table~\ref{tab:rq5_case_study_good_case_compare_with_llm-based_baseline}, compared to all LLM-based baselines, \ourapproach effectively reduced the number of errors almost across all categories for all studied LLMs. Specifically, compared to the best-performing baseline PE, \ourapproach demonstrated a reduction of 35.5\% to 76.5\% across all error categories. This indicates that \ourapproach can significantly enhance the model's ability to accurately identify and handle non one-to-one mapping dependency differences in incremental translation scenarios.

Additionally, compared to PE, Basic RAG showed similar or even higher error counts across these three dependency error categories for all studied LLMs. This suggests that even the prompt design in \ourapproach (i.e., the PE baseline) alone slightly improves the model's capability to handle repository-level context compared to the Basic RAG baseline, which is consistent with the conclusions in Section~\ref{sec:rq1}.

In terms of the Rule-based baseline, as shown in 
Table~\ref{tab:rq5_case_study_good_case_compare_with_rule-based_baseline}, C2Rust exhibited 3,307 Function Difference Misinterpretation errors across 138 out of 145 tasks, and 637 Data Type Differences Misinterpretation errors across 113 tasks, affecting 95.2\% and 77.9\% of the tasks, respectively. The reason is that rule-based methods operate at the syntax level and rely on one-to-one code mapping, making them unable to handle scenarios involving dependency differences. Specifically, as shown in Fig.~\ref{fig:bad_case_example_from_Rule-based_baseline}, the Rule-based baseline performs a direct one-to-one translation of dependency call statements without any adaptation, failing to handle differences in repository-level context.
However, C2Rust demonstrated the best performance in Variable Differences Misinterpretation. This is because C2Rust translates non-local variables by statically parsing the specific values of variables in the source language and directly using these values instead of variable names in the target language. While this approach effectively reduces compilation errors potentially caused by variable differences, it significantly compromises code readability and does not actually address repository-level differences between the source and target language versions.





\begin{table}
\caption{The Number of Top3 Error Causes of Dependencies Misuse of \ourapproach and Rule-based Baseline}
\centering
\begin{adjustbox}{width=0.85\linewidth}
        \begin{tabular}{@{}c|c|ccc}
            \hline
            \multirow{2}{*}{\textbf{Tech.}}  & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Error type}}                   \\ \cline{3-5} 
            & & \begin{tabular}[c]{@{}l@{}}\textbf{Function Differences}\\\textbf{Misinterpretation ↓}\end{tabular}  & \begin{tabular}[c]{@{}l@{}}\textbf{Data Type Differences}\\ \textbf{Misinterpretation ↓}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Variable Differences}\\\textbf{Misinterpretation ↓}\end{tabular} \\ \hline

            {C2Rust} & - &  3,307 & 637 & \textbf{26} \\ \hline
            \multirow{5}{*}{\textbf{\ourapproach}} 
                     & \claude &  26 & \textbf{0}&  48 \\ 
                     & \rdeepseek &  \textbf{23}& \textbf{0}&  31 \\ 
                     & \vdeepseek & 35 & \textbf{0} &  34 \\ 
                     & \qwenthreetwo &  112& \textbf{0} &  145 \\ 
                     & \qwenfourteen &  129 & \textbf{0} &   127 \\ \hline
        \end{tabular}
        \end{adjustbox}
\label{tab:rq5_case_study_good_case_compare_with_rule-based_baseline}
% \vspace{-10pt}
\end{table}

\begin{figure*}[b]
    % \vspace{-15pt}
    \centering
    \includegraphics[width=1\linewidth]{pictures/5_Result/Bad_Eample_From_Rule-based_Baseline.pdf}
    \caption{Failure Example From Rule-based baseline}
    \label{fig:bad_case_example_from_Rule-based_baseline}
    % \vspace{-10pt}
\end{figure*}





\subsubsection{Analysis of Failure Examples} 
In particular, we separately analyze the proportions of compilation errors and functional implementation errors in bad cases both before and after self-debugging. Furthermore, we classify compilation errors into finer-grained categories based on the taxonomy defined in RustRepoTrans~\cite{ou2024repository}. This analysis helps us identify which errors persist despite the triple-knowledge enhancement, as well as which errors can be easily fixed through self-debugging and which cannot. By doing so, we can pinpoint areas where future work should focus on improving LLM capabilities to further enhance performance in repository-level context code translation.

\begin{table}[t]
% \vspace{-20pt}
\caption{The Number of Each Error Causes of \ourapproach Before Self-debugging and After Self-debugging. One bad case can include more than one error}
\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{c|c|cc}
\hline
\multirow{2}{*}{Error Type}                                                   & \multirow{2}{*}{Error Causes}                       & \multicolumn{2}{c}{Number}                   \\ \cline{3-4} 
                                                                              &                                                     & \begin{tabular}[c]{@{}c@{}}Before \\ Self-debugging\end{tabular} & \begin{tabular}[c]{@{}c@{}}After \\ Self-debugging\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Functional \\ Implementation \\ Error\end{tabular} & -                                                   & 25                    &  27                    \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Compilation \\ Error\end{tabular}} & Data type Misinterpretation                         & 89                    & 54                   \\ \cline{2-4} 
                                                                              & Syntactic Differences Misinterpretation             & 0                     & 2                    \\ \cline{2-4} 
                                                                              & Function Differences Misinterpretation              & 309                   & 28                   \\ \cline{2-4} 
                                                                              & Variable Differences Misinterpretation              & 105                   & 16                   \\ \cline{2-4} 
                                                                              & Data Type Differences Misinterpretation             & 17                    & 9                    \\ \cline{2-4} 
                                                                              & Dependency Resolution Differences Misinterpretation & 0                     & 6                    \\ \cline{2-4} 
                                                                              & Function Signature Inconsistencies                  & 1                     & 0                    \\ \hline 
\end{tabular}
}
\label{tab:rq5_result}
% \vspace{-10pt}
\end{table}


\begin{figure*}[b]
    % \vspace{-15pt}
    \centering
    \includegraphics[width=1\linewidth]{pictures/5_Result/bad_case_example.pdf}
    \caption{Failure Example From \ourapproach}
    \label{fig:bad_case_example}
    % \vspace{-5pt}
\end{figure*}

Before self-debugging, compilation errors account for 79.3\%, which is already significantly lower than the 94.8\% reported in~\cite{ou2024repository} evaluating Basic LLM on RustRepoTrans. This indicates that triple knowledge enhancement effectively reduces issues such as dependency misuse, syntax misinterpretation, and syntactical difference confusion, thereby improving compilation rates.
As shown in Figure~\ref{fig:bug_type_propotion_before_debug}, the highest proportion of compilation error types is Function Differences Misinterpretation, accounting for 59.3\%, with a total of 309 occurrences (detailed in Table~\ref{tab:rq5_result}). Through case analysis, we found that \ourapproach sometimes fails to provide LLM with fully corrective knowledge, particularly when the dependencies in the source project do not exist in the target project.
as shown in Figure~\ref{fig:bad_case_example}, for the statement under translation: \texttt{W[0].copy(this)}, \ourapproach fails to provide the correct knowledge in both Target-Language Code Sample and Dependency Usage Example. This is because the dependency \texttt{copy} in the source project does not have a direct counterpart in the target project but should instead be implemented by using the built-in function \texttt{clone} in the target language. Since \texttt{copy} is not implemented in the target project, \ourapproach cannot retrieve a valid dependency usage example for it.
Additionally, a higher textual similarity does not always guarantee a functionally equivalent match. As a result, in some cases, the retrieved code sample fails to provide the correct translation guidance. Therefore, even though Successful Translation Function Pair provides a correct example, the noise introduced by the other two types of knowledge misleads the LLM, ultimately leading to an incorrect translation.

After self-debugging, the proportion of compilation errors further decreased to 59.7\%. Notably, the most frequent compilation error before self-debugging—Function Differences Misinterpretation—dropped from 59.3\% to 24.3\%, with occurrences drastically reducing from 309 to just 28. This suggests that many of the existing shortcomings in \ourapproach can be effectively addressed by self-debugging.
It is important to note that Data Type Misinterpretation did not show a significant reduction after self-debugging. This is most likely because the target language (Rust) in the evaluated dataset is a low-resource language with stringent compile-time checks enforced by its ownership model and borrow checker. As a result, LLMs struggle with Rust-specific constraints in ways that cannot be easily mitigated by simply providing code samples. We will further explore and address this challenge in future work. 

\finding{\ourapproach fails to provide LLM with fully corrective knowledge in certain cases, such as when the dependencies in the source project do not exist in the target project. However, many of the existing shortcomings in \ourapproach can be effectively addressed by self-debugging.}

\begin{figure}[tbp]
% \vspace{-0.7em}
    \centering
    % 第1张图
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{pictures/5_Result/bug_type_propotion_before_debug.pdf}
        \caption{Distribution of Error Causes of \ourapproach before self-debugging}
        \label{fig:bug_type_propotion_before_debug}
        
    \end{minipage}
    \hspace{0.02\textwidth} % 控制水平间距
    % 第2张图
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{pictures/5_Result/bug_type_propotion_after_debug.pdf}
        \caption{Distribution of Error Causes of \ourapproach after self-debugging}
        \label{fig:bug_type_propotion_after_debug}
    \end{minipage}
% \vspace{-15pt}
\end{figure}




==> sections/app/knowledge_base_construction.tex <==
% \vspace{-5pt}
\subsection{Translation Knowledge Base Construction}
\label{sec:phase1}


In \ourapproach, the translation knowledge base consists of three parts: dependency usage examples from the repository being translated (in Section \ref{sec:dependency_calling_examples}), target-language code samples from existing projects (in Section \ref{sec:target_language_code_examples}), and translation pair examples from previous successful translation (in Section~\ref{sec:successful_translation_pairs}), which are aimed to enhance LLM's ability to correctly recognize and invoke dependencies, understanding of target language's syntax, and capability to identify syntax differences. 

\subsubsection{Dependency Usage Examples Extraction}
\label{sec:dependency_calling_examples}
% 可能放到introduction部分
% LLMs在进行repo-level的代码任务时，往往需要处理复杂的context and dependencies， 但是模型通常
% 由于同一个依赖项在同一个项目中通常会被多次调用，其他地方的调用方式会对目标函数内调用方式具有参考意义。具体来说，当作用域相同时，对于同一个依赖项具有相同的调用路径和相同类型的传入参数。当作用域不同时，对于同一依赖项具有相似的调用路径和相同类型的传入参数。因此对于每一个翻译任务中涉及的每一个依赖项会从当前项目中与当前目标函数所处的作用域相同的代码中提取出对应的依赖项调用语句，构成dependency calling examples，以此增强LLMs正确识别并调用依赖项的能力。

Since the same dependency is often called multiple times within the same project, the way a dependency is called elsewhere in the project can serve as a useful reference for its usage in the target function. Specifically, when the scope is the same, the same dependency will have the same call path and identical types of input parameters. When the scope differs, the call path will be similar and the input parameters will still be of the same type. 
Therefore, for each dependency involved in a translation task, we extract the corresponding dependency call statements from the code in the current project that shares the same scope as the target function. If multiple call statements are found, only the first occurrence is retained as the example.
Specifically, by utilizing tree-sitter~\cite{tree-sitter}, we extract function dependencies by identifying \textit{call\_expression} nodes to retrieve all function invocation statements. These statements are then filtered based on the names of the target function dependency, obtaining the required dependency invocation statements.
For variable dependencies, we extract code execution statements and filter them according to the names of the target variable dependency, thereby obtaining the corresponding variable dependency invocation statements.
Ultimately, for each dependency, we constructed the corresponding dependency usage examples with \texttt{[source code of dependency]} and \texttt{[usage example]} (if no corresponding invocation statement was retrieved, \texttt{[usage example]} is set to empty). These extracted statements form the dependency usage examples, enhancing the LLM's ability to correctly identify and invoke dependencies.

This component is self-evolving by continuously performing the dependency extraction operations mentioned before \colortext{to extract dependency usage examples from successfully translated code or from components that have been refactored, or updated manually by developers that has been subsequently integrated into the project's repository context during translation process.}

% \vspace{-6pt}
\subsubsection{Target-language Code Samples Extraction}
\label{sec:target_language_code_examples}
Existing work has shown that providing the model with code snippets similar to the target code as a reference improves the quality of generated code in code generation tasks~\cite{fan2024surveyragmeetingllms}. 
Since code implementing the same functionality often uses similar function names and variable names, leading to higher textual similarity~\cite{zhong2010mining}, retrieving the target-language code with the highest textual similarity to the function under translation allows us to effectively identify code samples from similar-domain projects that implement comparable functionality.
These code samples could help improve translation as well.
To simulate the most comprehensive reference code for the target language currently available, we obtained open source projects on GitHub that were created before March 31, 2022, from the The Stack dataset~\cite{Kocetkov2022TheStack} to directly assess function-level code samples. Then, using the official GitHub API, we crawled open source projects created after March 31, 2022, based on the condition \textit{`language: \$target\_language created:2022-04-01..2025-02-01'}, and then used tree-sitter~\cite{tree-sitter} to extract function from source file. 
% We set the \$target\_language to Rust, consistent with the evaluation dataset~\cite{ou2024repository} (in Section \ref{sec:benchmark}).
To prevent potential data leakage in the knowledge base, we remove all projects with the same name as those involved in evaluation benchmark~\cite{ou2024repository}, regardless of whether their creators are the same, considering the possibility of project forks.
These two parts together form the General Projects of the knowledge base, containing a total of 113,882,369 target language code examples from 671,240 projects, which are used to enhance the code generated by the LLM to better conform to the syntax requirements of the target language.

This component is self-evolving by automatically detecting and downloading newly added target-language projects from GitHub with pre-configured update interval.

% Completed:
% \todo{the projects in similar domian could help translation as well.}
% \todo{add XXX projects in total.}
% \todo{describe how to get code samples from projects.}
% \todo{describe how this knowledge could be evolved, new project, new commit, new translated code repository}



% 这部分是不是放在introduction会比较好
% Dividing complex code tasks into simpler sub-tasks based on the divide-and-conquer principle has been shown to effectively improve the performance of LLMs on complex tasks \cite{wang2024hits}. Moreover, in complex code translation scenarios, models tend to perform one-to-one translation at the statement level within the target function, rather than understanding the functionality of the source function and then implementing it according to the target language's syntax and existing dependencies. This translation approach is prone to overlooking potential syntactic and dependency differences between the source and target languages, which can lead to compilation errors. As shown in Figure \ref{fig:motivation_example_syntax_diff}, due to syntactic differences between the source and target languages (e.g., in C, null pointer checks are required before using pointer variables, whereas Rust's non-Option type variables do not require such checks), LLMs must accurately identify that the null pointer check in the source language is unnecessary in the target language. However, when translating at the function level, the complexity of the task often prevents the model from precisely identifying this syntactic difference and skipping the check statements in the source language. When the function-level translation task is composed into slice-level sub-tasks, the model’s ability to recognize syntactic differences is significantly enhanced (see Section \ref{sec:result}).
% Because the check statements involved in syntactic differences are typically implemented using if-else statements \cite{ou2024repository}, and loop constructs are commonly used as delimiters when partitioning the functionality of a function \cite{?}, after extracting all functions from the collected projects using Tree-sitter \cite{tree-sitter}, we split the function-level code into slice-level code by using if-else and loop statements as delimiters resulting in \todo{xxx} slice-level code snippets. 

%\begin{figure}
%    \centering
%    \includegraphics[width=1\linewidth]{pictures/3_Approach/motivation_example_syntax_diff.pdf}
%    \caption{difference with translating in function-level and slice-level}
%    \label{fig:motivation_example_syntax_diff}
%\end{figure}




% \vspace{-5pt}
\subsubsection{Successful Translation Function Pair Examples Collection}
\label{sec:successful_translation_pairs}
Providing the model with information of the same category as the target task could maximize its performance on the current task. However, due to the scarcity of existing repository-level context code translation datasets~\cite{ou2024repository}, it is difficult to obtain a large number of high-quality function-level equivalence pairs to construct successful translation function pairs base, for repository-level context. Therefore, we collect successful translation function pairs during the translation process and add them to the knowledge base, constructing the successful translation function pairs knowledge base, which are used to enhance model's ability to recognize syntactic differences when performing code translation tasks.

This component is self-evolving by constantly extracting successful translation function pairs, which has been evaluated by test cases, from prior translation history.

==> sections/app/retrieval.tex <==
% \vspace{-5pt}
\subsection{Translation Knowledge Retrieval}
\label{sec:phase2}
The input of the repository-level context code translation task consists of three parts: the source code of the function under translation, the function signature of target function, and the target function dependencies.
For a given repository-level context code translation task, \ourapproach retrieves relevant translation knowledge from the constructed translation knowledge to construct translation prompt (as shown in Figure~\ref{fig:prompt_example}) base in a three-step retrieval process: focal function and dependencies extraction, candidate knowledge retrieval, candidate knowledge re-ranking.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{pictures/3_Approach/necessity_of_unixcoder_resort.pdf}
%     \caption{Example of BM25 shortcomings}
%     \label{fig:necessity_of_unixcoder_resort}
% \end{figure}
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{pictures/3_Approach/prompt_example.pdf}
    % \vspace{-18pt}
    \caption{Overview of Prompt Construction (using C to Rust as example)}
    \label{fig:prompt_example}
    % \vspace{-13pt}
\end{figure*}

% \vspace{-3pt}
\subsubsection{Focal Function and Dependencies Extraction}
For each repository-level context code translation task, \ourapproach follows the segmentation method described in the evaluated dataset to extract different parts of the translation task. With pattern matching, it separately extracts the source code of the function under translation and its corresponding dependencies.
The source code of the function under translation is used to retrieve target-language code examples and successful translation function pairs (details in Section~\ref{sec:candidate_knowledge_retrieval}). Meanwhile, the dependencies are matched against the \texttt{[source code of dependency]} in the Dependency Usage Examples and the corresponding \texttt{[usage example]} is extracted as the dependency usage example for the dependency.

% For each repository-level context code translation task, \ourapproach first extracts the focal function and its corresponding dependencies separately, which are used to retrieve target-language code examples and successful translation function pairs, as well as retrieve dependency usage examples. 
% Completed:
% \todo{this part is not clear}


% For each repository-level context code translation task, \ourapproach first decomposes the function-level source code into slice-level segments with the same rules described in the knowledge base construction (Section \ref{sec:phase1}). However, the difference is \ourapproach adopts LLMs instead of rule-based to split the source code in order to generate natural language descriptions of functionality summaries for each function and slice at the same time. This is because, compared to code snippets, natural language descriptions allow the model to better understand the specific functionality of the current function \cite{DBLP:journals/corr/abs-2406-11147}, thus improving the consistency between the generated code and the source code. 

% To help the LLM understand the decomposition task, we design the Chain-of-thought strategy, leading the LLM to work step by step. First, the LLM is asked to summarize the focal function. Second, to understand the slice in detail, we ask LLM to describe the functionality of the slice without concrete code elements and replicate the corresponding code statements without changing anything. Besides, we use oneshot prompting here, providing a hand-craft example according to different source language illustrating how to decompose a function into several slices. Based on the previous steps of analysis and prompt engineering skills, the LLM is required to decompose the focal function into slices. 

% After segmentation, the resulting function summary, source code of the slice, and slice summary are served as inputs for the subsequent Knowledge-Augmented Code Translation phase, with the source code of the slice serving as input for candidate knowledge retrieval.

% \vspace{-3pt}
\subsubsection{Candidate Knowledge Retrieval}
\label{sec:candidate_knowledge_retrieval}
For each focal function to be translated, \ourapproach adopts BM25~\cite{robertson1994some}, a method widely used in search engines due to its efficiency and effectiveness~\cite{achiam2023gpt}, based on Elasticsearch~\cite{elasticsearch}, an open source high-performance, RESTful search and analytics engine, to retrieve the top n, where n = 100 for target-language code sample and n = 10 for successful translation function pairs in our experiments, knowledge items for each query function. 
In the field of information retrieval, BM25 calculates the similarity score between a query \( q \) and the documentation \( d \) for retrieval. BM25 computes the similarity score according to the following Equation \ref{equation:BM25}, where \( f(w_i, q) \) is the word \( w_i \)'s term frequency in query \( q \), and \( IDF(w_i) \) is the inverse document frequency of word \( w_i \). The hyperparameters \( k \) (where \( k = 1.2 \) and \( b = 0.75 \)) are employed to normalize term frequencies and control the influence of document length. Prior to calculating the BM25 similarity, both the query and the retrieval documentation undergo essential preprocessing procedures, including tokenization, lemmatization, and stop word removal~\cite{ccaugatayli2015effect}.

% \vspace{-5pt}
{\footnotesize
\begin{equation}
\text{Sim}_{BM25}(q, d) = \sum_{i=1}^{n} \frac{IDF(w_i) \times f(w_i, q) \times  (k+1)}{f(w_i, q) + k \left( 1-b+b \times \frac{|q|}{avgdl} \right)} )
\label{equation:BM25}
\end{equation}
}


\subsubsection{Candidate knowledge Re-ranking}
Although BM25 performs excellently in text-based similarity calculations, it struggles to effectively identify noise, such as comments, and other critical information within code, such as the Abstract Syntax Tree (AST). Therefore, \ourapproach employs UniXcoder~\cite{DBLP:conf/acl/GuoLDW0022}, a unified cross-modal pre-trained model for programming languages, to re-rank the retrieved knowledge items by calculating cosine similarity. The top n, where n = 2 for target-language code sample (will be discussed further in Section~\ref{sec:rq3}) and n = 1 for successful translation function pairs in our experiments candidate knowledge items with the highest UniXcoder scores are selected as the final knowledge items to be provided to the LLM-based code translation.



% Completed:
% \todo{describe in more details. Using Cosine similarity calculated by Unixcoder to rerank? do we filter top-1 code snippet with low similarity? }

==> sections/app/translation.tex <==
\subsection{Knowledge-Augmented Code Translation}
\label{sec:phase3}
We first utilize LLMs to perform translation based on retrieved triple translation knowledge, obtaining initial results, and then apply LLM-based code repair to fix any identified issues.

\parabf{LLM-based code translation.} Based on the retrieved translation knowledge items, \ourapproach leverages LLMs to translate code from the source language to the target language. The prompt design (as shown in Figure~\ref{fig:prompt_example}) adopts an LLM-friendly format: markdown~\cite{prompt_engineering}, and we also design the Chain-of-Thought strategy~\cite{wei2023chainofthoughtpromptingelicitsreasoning}, guiding the LLM to translate the function step by step. Firstly, the LLM is asked to confirm the functionality to be implemented by the current function. Second, to understand the differences between the source and target programming languages, such as the differences of dependencies, syntax and available local variables in detail, we apply the recitation technique, asking the LLM to enumerate all used dependencies and local variables as well as distinguish the syntax differences. Finally, LLM translates the focal function based on the functionality implemented by the function, the dependencies used, and the syntax differences.

\begin{figure*}[b]
    \centering
    \includegraphics[width=0.8\linewidth]{pictures/3_Approach/repair_prompt.pdf}
    % \vspace{-10pt}
    \caption{Prompt For Code Repair}
    \label{fig:prompt_code_repair}
    % \vspace{-13pt}
\end{figure*}

\parabf{LLM-based code repair.} The code translated by LLMs may contain simple syntax errors (e.g., performing mutable operations on immutable variables). Previous work~\cite{deligiannis2024rustassistant} has shown that LLMs can repair certain errors in code using compiler error messages. After translation, \ourapproach provides the LLM with specific instructions to leverage error message and iteratively refine translation results that fail testing due to compilation or functional errors. While this process can be conducted for multiple iterations, our implementation limits it to one iteration for cost-effectiveness. This approach further improves translation accuracy and assesses the percentage of erroneous translations that can be successfully repaired. The prompt used for code repair is shown as Fig.~\ref{fig:prompt_code_repair}

